Logical Consistency of Large Language Models in Fact-checking

In recent years, large language models (LLMs) have demonstrated significant success in performing varied natural language tasks such as language translation, question-answering, summarizing, fact-checking, etc. Despite LLMs' impressive ability to generate human-like texts, LLMs are infamous for their inconsistent responses - a meaning-preserving change in the input query results in an inconsistent response and attributes to vulnerabilities of LLMs such as hallucination. Consequently, existing research focuses on simple paraphrasing-based consistency assessment of LLMs, and ignores complex queries that necessitate an even better understanding of logical reasoning by an LLM. Our work therefore addresses the logical inconsistency of LLMs under complex logical queries with primitive logical operators, e.g., negation, conjunction, and disjunction. As a test bed, we consider retrieval-augmented LLMs on a fact-checking task involving propositional logic queries from knowledge graphs (KGs). Our contributions are threefold. Benchmark: We introduce three logical fact-checking datasets over KGs for community development towards logically consistent LLMs. Assessment: We propose consistency measures of LLMs on propositional logic queries and demonstrate that existing LLMs lack logical consistency, especially on complex queries. Improvement: We employ supervised fine-tuning to improve the logical consistency of LLMs on the complex fact-checking task with KG contexts. We have made our source code and benchmarks available.

==> 3-consistency_extra.tex <==
\clearpage
\bghosh{Will be removed}
\section{Measuring LLM Consistency using First-order Logic Queries}


Consider a triple $ T =  (u, r, v) $ where $ u, v \in \mathcal{V} $, $ T \in \mathcal{T} $ and the corresponding relation $ r(u, v) $. 


LLM generally operates on a natural language. Let $ \phi(r(u, v)) $ be a natural language representation of the relation $ r(u, v) $. Formally, $ \phi(T) \equiv \phi(r(u, v)) $, that is we flexibly interchange between a triple and a relation.

\begin{example}
    \normalfont
    Consider the relation $ r = \texttt{participant} $, $ u = \text{2008 Olympics} $, and $ v = \text{Usain Bolt} $. Then $ \phi(r(u, v)) $ can simply be a line with `$ \mid $' separated tuples: (2008 Olympics $ \mid $ \texttt{participant} $ \mid $ Usain Bolt).
\end{example}

An LLM constitutes a function $ \texttt{LLM}(\phi(r(u, v)), c) $ which takes input as the natural text for the relation $ r $ and context $ c $. Context can also be provided from a KG as a set of $ n $ triples $ \mathbf{T} = \{T\}_{i=1}^n $ and $ c = \{\phi(T)\}_{i=1}^n $. We provide in-context examples as context $ c $.



The LLM response can be a binary value, meaning that it can either confirm a relation or cannot confirm it, irrespective of how the context $ c $ is provided. 

\[
    \texttt{LLM}(\phi(r(u, v)), c) \in \{\text{True, False}\}
\]


\begin{example}
    \normalfont
    Let the context $ c = \{ (\text{Usain Bolt} \mid \texttt{GoldMedalAwarded}) \mid \text{2008 Onlympics} \}$. If the LLM can conceptualize the context, then the response $ \texttt{LLM}(\phi(\texttt{participant}(\text{2008 Olympics}, \text{Usain Bolt}), c) = \text{True} $.
\end{example}

The accuracy of $ \texttt{LLM} $ is the expectation that the LLM response matches with the provided relation. 

\textcolor{red}{[AK: In the previous example, the LLM response does not ``exactly'' match with the provided relation, e.g., \texttt{GoldMedalAwarded} vs. \texttt{participant}. How to clarify this appropriately?]}

\[
    \mathbb{E}_{r(u, v)} \mathds{1}(\texttt{LLM}(\phi(r(u, v)), c) = r(u, v))
\]

To avoid notational clutter, we use $ \texttt{LLM}(r(u, v)) $ to denote $ \texttt{LLM}(\phi(r(u, v)), c) $ when it is clear from the context.

\subsection{Negation.}

\textbf{Single answer}: Consider a triple $ T' = (u, r, v') $ where $ v \ne v' $ and $ v' \in \mathcal{V} $. Thus, $ r(u, v') $ is a negative query concerning $ r(u, v) $ since the object entity is different and $r(u, v) = \neg r(u, v')$. The LLM is consistent for the negation query if $ \texttt{LLM}(r(u, v)) = \neg \texttt{LLM}(r(u, v')) $. 

\textcolor{red}{[AK: Instead of single answer vs. multiple answer, can we say more formally, e.g., injective/ non-injective, one-to-one/ one-to-many relation $r$?]}


\textbf{Multiple answers}: We extend to the case where $ r(u, v_i) = \text{True} $ for all $ v_i \in \mathbf{V} $. In this case, the negative query is $ r(u, v') $ where $ v' \notin \mathbf{V} $.  Then, the LLM is consistent with the negative query if $ \forall i. \texttt{LLM}(r(u, v_i)) = \neg \texttt{LLM}(r(u, v')) $.

\begin{example}
    \normalfont
    We consider a relation $ \texttt{participant}(\text{2008 Olympics}, \text{Usain Bolt}) $. A negative relation be $ \texttt{participant}(\text{2008 Olympics}, \text{Maradona}) $. The LLM response of the positive and the negative query be complementary. 
\end{example}



\subsection{Conjunction}

Let $ r_i(u, v_i) $ and $ r_j(u, v_j) $ are two relations. Consider a conjunctive relation $ r_i(u, v_i) \wedge r_j(u, v_j) $. LLM is consistent on conjunctive queries when 
\[
    \texttt{LLM}(r_i(u, v_i) \wedge r_j(u, v_j)) = \texttt{LLM}(r_i(u, v_i)) \wedge \texttt{LLM}(r_j(u, v_j))
\]


\begin{example}
    \normalfont
    Let two relations with same subject entity be $ \texttt{participant}(\text{2008 Olympics}, \text{Usain Bolt}) $ and $ \texttt{hostCountry}(\text{2008 Olympics}, \text{China}) $. Then the conjunctive query in the natural text is `Usain Bolt participated in the 2008 Olympics, which was held in China'. An LLM that outputs True to the conjunctive query should output True for each query. 
\end{example}


\subsection{Disjunction}

Let $ r_i(u, v_i) $ and $ r_j(u, v_j) $ are two relations. Consider a conjunctive relation $ r_i(u, v_i) \vee r_j(u, v_j) $. LLM is consistent on conjunctive queries when 
\[
    \texttt{LLM}(r_i(u, v_i) \vee r_j(u, v_j)) = \texttt{LLM}(r_i(u, v_i)) \vee \texttt{LLM}(r_j(u, v_j))
\]

\begin{example}
    \normalfont
    \textcolor{blue}{[BG: Find a meaningful disjunctive example.]}
\end{example}

\textcolor{red}{[AK: So far, we defined correctness, how to formally define consistency?]}

\clearpage
\section{Consistency Revised}
\subsection{Negation Consistency of a Single Chain Query.} A single chain query is $ r(v_1, v_2) $ which relates the subject entity $ v_1 $ with the object entity $ v_2 $ via the relation $ r $. Such a relation is derived from a knowledge graph. For a one to one relation $ r $, the negation query is $ r(v_1, v'_2) $ where $ v_2 \ne v'_2 $. We defer the analysis for one-to-many relations at the end of this section. The LLM response $ \mathtt{LLM}: \mathcal{R} \rightarrow \{0, 1\} $ is a binary function that either validates or invalidates the input relation $ r \in \mathcal{R} $.


\begin{figure}
	\centering
	\begin{tikzpicture}[node distance=2cm]
		
		
		\node[circle, draw] (v_1) at (0, 0) {$v_1$};
		\node[circle, draw] (v_2) at (2, 0) {$v_2$};
		
        \draw[arrow](v_1) -- (v_2) node [pos=0.5, above] {$r_1$};;
		
	\end{tikzpicture}
    \caption{A single chain query}
\end{figure}

\begin{lemma}
    For a single chain query $ r(v_1, v_2) $ and a corresponding negative query $ r(v_1, v'_2) $ where $ v_2 \ne v'_2 $, the LLM response is correct when the following two cases are satisfied.
    \begin{align}
        \mathtt{LLM}(r(v_1, v_2)) = 1 \\
        \mathtt{LLM}(r(v_1, v'_2)) = 0
    \end{align}
\end{lemma} 
Intuitively, the LLM is expected to validate any fact such as $ r(v_1, v_2) $ from the knowledge graph and invalidate any alternative fact such as $ r(v_1, v'_2) $ from the same knowledge graph.
Traditional precision ($ \frac{TP}{TP+FP} $), recall ($ \frac{TP}{TP+FN} $), or accuracy ($ \frac{TP + TN}{P + N} $) notions can be applied to determine the correctness of the LLM response. Here $ r(v_1, v_2) $ and $ r(v_1, v'_2) $ constitute positive and negative classes respectively in the traditional sense of machine learning classification.


\begin{lemma}
    For a single chain query $ r(v_1, v_2) $ and a corresponding negative query $ r(v_1, v'_2) $ where $ v_2 \ne v'_2 $, the LLM response is logically consistent when 

    \begin{align}
        &\mathtt{LLM}(r(v_1, v_2)) \ne \mathtt{LLM}(r(v_1, v'_2))\\
        \Rightarrow & 
        \begin{cases}
            \mathtt{LLM}(r(v_1, v'_2)) = 0 & \text{if}\quad   \mathtt{LLM}(r(v_1, v_2)) = 1\\
            \mathtt{LLM}(r(v_1, v'_2)) = 1 & \text{otherwise}
        \end{cases}
    \end{align}
\end{lemma}

Therefore, an LLM is logically consistent in two cases: (i) when it is correct and (ii) when it is incorrect but makes an incorrect response to the alternative fact $ r(v_1, v'_2) $. 


\subsection{Conjunctive Consistency of a Two-chain Query.} A two-chain query is a simple form of conjunctive query. Formally, a two-chain query 
\begin{align}
    r_1(v_1, v_2) \wedge r_2(v_2, v_3)
\end{align} comprises of two relations $ r_1, r_2 $ joining three entities $ v_1, v_2, v_3 $ in a chain. Since a two-chain query has three entities, there are three possible ways to construct a corresponding negative query in the following.


\begin{figure}
	\centering
	\begin{tikzpicture}[node distance=2cm]
		
		
		\node[circle, draw] (v_1) at (0, 0) {$v_1$};
		\node[circle, draw] (v_2) at (2, 0) {$v_2$};
        \node[circle, draw] (v_3) at (4, 0) {$v_3$};
		
        \draw[arrow](v_1) -- (v_2) node [pos=0.5, above] {$r_1$};;
        \draw[arrow](v_2) -- (v_3) node [pos=0.5, above] {$r_2$};;
		
	\end{tikzpicture}
    \caption{A two-chain conjunctive query}
\end{figure}

\begin{align}
    r_1(v'_1, v_2) \wedge r_2(v_2, v_3), v_1 \ne v'_1\\
    r_1(v_1, v'_2) \wedge r_2(v'_2, v_3), v_2 \ne v'_2\\
    r_1(v_1, v_2) \wedge r_2(v_2, v'_3), v_3 \ne v'_3
\end{align}

\begin{lemma}
    Consider six entities $ \{v_1, v_2, v_3, v'_1, v'_2, v'_3\} $ where $ v_1 \ne v'_1 $, $ v_2 \ne v'_2 $, $ v_3 \ne v'_3 $ and two relations $ \{r_1, r_2\} $. An LLM response is correct for a two-chain conjunctive query $ r_1(v_1, v_2) \wedge r_2(v_2, v_3) $ when the following four cases are satisfied.

    \begin{align}
        \mathtt{LLM}(r_1(v_1, v_2) \wedge r_2(v_2, v_3)) = 1\\
        \mathtt{LLM}(r_1(v'_1, v_2) \wedge r_2(v_2, v_3)) = 0\\
        \mathtt{LLM}(r_1(v_1, v'_2) \wedge r_2(v'_2, v_3)) = 0\\
        \mathtt{LLM}(r_1(v_1, v_2) \wedge r_2(v_2, v'_3)) = 0
    \end{align}
\end{lemma}

Intuitively, for a two-chain query response to be correct, the LLM must validate a given fact from a knowledge graph and all possible alternative facts from the same knowledge graph.


\begin{lemma}
    Consider six entities $ \{v_1, v_2, v_3, v'_1, v'_2, v'_3\} $ where $ v_1 \ne v'_1 $, $ v_2 \ne v'_2 $, $ v_3 \ne v'_3 $ and two relations $ \{r_1, r_2\} $. An LLM response is logically consistent for a two-chain conjunctive query $ r_1(v_1, v_2) \wedge r_2(v_2, v_3) $ when the following condition is satisfied.

    \small
    \begin{align*}
        &\mathtt{LLM}(r_1(v_1, v_2) \wedge r_2(v_2, v_3)) = \mathtt{LLM}(r_1(v_1, v_2)) \wedge \mathtt{LLM}(r_2(v_2, v_3))
    \end{align*}
    \normalsize

    Breaking down to \red{correct and incorrect} LLM responses, the consistency criteria for a two-chain conjunctive query is in the following.


    \begin{align*}
        \begin{cases}
            \begin{aligned}
                &\mathtt{LLM}(r_1(v_1, v_2)) = 1  \;\wedge & \text{if} \;\; \mathtt{LLM}(r_1(v_1, v_2) \wedge r_2(v_2, v_3)) = 1 \\
                &\mathtt{LLM}(r_2(v_2, v_3)) = 1 & \\
                \\
                &\mathtt{LLM}(r_1(v_1, v_2)) = 0  \;\vee & \text{if} \;\; \mathtt{LLM}(r_1(v_1, v_2) \wedge r_2(v_2, v_3)) = 0 \\
                &\mathtt{LLM}(r_2(v_2, v_3)) = 0 & \\
            \end{aligned}
        \end{cases}
    \end{align*}


    
    
\end{lemma}

Therefore, the consistency condition for two-chain conjunctive query reduces to validating LLM responses on single-chain queries, which we can further be validated for negation-based consistency.

\subsection{Conjunctive Consistency of a Two-branch Query.}
A two-branch conjunctive query has the following form.
\begin{align}
    r_1(v_1, v_2) \wedge r_2(v_3, v_2),
\end{align}


\begin{figure}
	\centering
	\begin{tikzpicture}[node distance=2cm]
		
		
		\node[circle, draw] (v_1) at (0, 0) {$v_1$};
		\node[circle, draw] (v_2) at (2, -1) {$v_2$};
        \node[circle, draw] (v_3) at (0, -2) {$v_3$};
		
        \draw[arrow](v_1) -- (v_2) node [pos=0.5, above] {$r_1$};;
        \draw[arrow](v_3) -- (v_2) node [pos=0.5, above] {$r_2$};;
		
	\end{tikzpicture}
    \caption{A two-branch conjunctive query}
\end{figure}

where in both relations, the object entity $ v_2 $ is common. \red{A two-branch conjunctive query can be reduced to a two-chain conjunctive query via the following equivalent relation: $ r_2(v_3, v_2) \equiv r'_2(v_2, v_3) $. Here $ r'_2 $ is a reverse relation to $ r_2 $. Therefore, the correctness and logical consistency check of a two-branch query can be reduced to an equivalent two-chain conjunctive query.} 


\subsection{Disjunctive Consistency of a Two-branch Query.}

A two-branch disjunctive query has the following form.
\begin{align}
    r_1(v_1, v_2) \vee r_2(v_3, v_2)
\end{align}

\begin{figure}
	\centering
	\begin{tikzpicture}[node distance=2cm]
		
		
		\node[circle, draw] (v_1) at (0, 0) {$v_1$};
		\node[circle, draw] (v_2) at (2, -1) {$v_2$};
        \node[circle, draw] (v_3) at (0, -2) {$v_3$};
		
        \draw[arrow](v_1) -- (v_2) node [pos=0.5, above] {$r_1$};;
        \draw[arrow](v_3) -- (v_2) node [pos=0.5, above] {$r_2$};;
		
	\end{tikzpicture}
    \caption{A two-branch disjunctive query}
\end{figure}

 Here, the objective entity $ v_2 $ is shared across two relations $ \{r_1, r_2\} $. A disjunctive query has two equivalent positive relations. 

 \begin{align*}
      r_1(v_1, v_2) \vee r_2(v_3, v_2)
     &\equiv  r_1(v'_1, v_2) \vee r_2(v_3, v_2) \\
     &\equiv r_1(v_1, v_2) \vee r_2(v'_3, v_2)
 \end{align*}

 where $ v_1 \ne v'_1 $ and $ v_3 \ne v'_3 $. In addition, the negation of the disjunctive query is $ r_1(v_1, v'_2) \vee r_2(v_3, v'_2) $ where the shared object entity $ v_3 \ne v'_3 $. 

\begin{lemma}
Consider six entities $ \{v_1, v_2, v_3, v'_1, v'_2, v'_3\} $ where $ v_1 \ne v'_1 $, $ v_2 \ne v'_2 $, $ v_3 \ne v'_3 $ and two relations $ \{r_1, r_2\} $. An LLM response is correct for a two-chain disjunctive query $ r_1(v_1, v_2) \vee r_2(v_3, v_2) $ when the following four cases are satisfied.

\begin{align}
        \mathtt{LLM}(r_1(v_1, v_2) \vee r_2(v_3, v_2)) = 1\\
        \mathtt{LLM}(r_1(v'_1, v_2) \vee r_2(v_3, v_2)) = 1\\
        \mathtt{LLM}(r_1(v_1, v_2) \vee r_2(v'_3, v_2)) = 1\\
        \mathtt{LLM}(r_1(v_1, v'_2) \vee r_2(v_3, v'_2)) = 0
    \end{align}

    
\end{lemma}


\begin{lemma}
    Consider six entities $ \{v_1, v_2, v_3, v'_1, v'_2, v'_3\} $ where $ v_1 \ne v'_1 $, $ v_2 \ne v'_2 $, $ v_3 \ne v'_3 $ and two relations $ \{r_1, r_2\} $. An LLM response is logically consistent for a two-chain disjunctive query $ r_1(v_1, v_2) \vee r_2(v_3, v_2) $ when the following condition is satisfied.

    \small
    \begin{align*}
        &\mathtt{LLM}(r_1(v_1, v_2) \vee r_2(v_3, v_2)) = \mathtt{LLM}(r_1(v_1, v_2)) \vee \mathtt{LLM}(r_2(v_3, v_2))
    \end{align*}
    \normalsize


    Breaking down to \red{correct and incorrect} LLM responses, the consistency criteria for a disjunctive two-branch query is in the following.


    \begin{align*}
        \begin{cases}
            \begin{aligned}
                &\mathtt{LLM}(r_1(v_1, v_2)) = 1  \;\vee & \text{if} \;\; \mathtt{LLM}(r_1(v_1, v_2) \vee r_2(v_3, v_2)) = 1 \\
                &\mathtt{LLM}(r_2(v_3, v_2)) = 1 & \\
                \\
                &\mathtt{LLM}(r_1(v_1, v_2)) = 0  \;\wedge & \text{if} \;\; \mathtt{LLM}(r_1(v_1, v_2) \vee r_2(v_3, v_2)) = 0 \\
                &\mathtt{LLM}(r_2(v_3, v_2)) = 0 & \\
            \end{aligned}
        \end{cases}
    \end{align*}
    
\end{lemma}


Si

\clearpage


 


\textcolor{red}{[AK: The following lemma should change since we are not considering multiple choice questions. We consider questions that can have multiple correct answers. In addition to the lemma, we should also give a measure to quantify it.- @Bishwa]}




\blue{[BG: Need to update the remaining part in Section 3.1.]}
\begin{lemma}[Negation]
For binary choices, such as $ C = \{c, \neg c\} $, the LLM is \textbf{logically consistent} if the following holds true.
    \begin{align}
        r(p) = \neg r(\bar{p})
    \end{align}     
\end{lemma}

\textcolor{red}{[AK: The following example should change. Perhaps consider one ground-truth example from our dataset. - @Bishwa]}
     
\begin{example}
\normalfont
\begin{align*}
    &q = \texttt{The ceramic vase was \dgreen{less} flexible than the plastic ball so it was}\\
    &\bar{q} = \texttt{The ceramic vase was \red{more} flexible than the plastic ball so it was}\\
    &C = \{\texttt{more breakable, less breakable}\}
\end{align*}
Let $ r(q, C) =  \texttt{more breakable} $. The LLM is logically consistent if $ r(\bar{q}, C) =  \texttt{less breakable} $ and vice versa.
\end{example}


\begin{lemma}[Negation]
For multiple choices $ |C| \ge 3 $, the LLM is \textbf{logically consistent} if the following holds true.
    \begin{align}
        r(p) \ne  r(\bar{p})
    \end{align}     
\end{lemma}

\begin{example}
\normalfont
    Consider the following multi-choice:
    \begin{align*}
        &C = \{\texttt{more breakable, less breakable, equally breakable}\}\\
        &r(q, C) =  \texttt{more breakable}\\
        &r(\bar{q}, C) \in \{\texttt{less breakable, equally breakable}\}
    \end{align*}
\end{example}


Let $ r(q, C) $ return a set of choices. For a unique and single answer, we consider $ r(q, C) $ as a singleton set.

\subsection{Conjunction.}
Let $ T_i = (u, r_i, v_i) $ and $ T_j = (u, r_j, v_j) $ are two triples where $ T_i, T_j \in \mathcal{T} $. Consider a conjunctive relation $ r = r_i(u, v_i) \wedge r_j(u, v_j) $.


\blue{[BG: Need to update the remaining part in Section 3.1.]}

\begin{lemma}[Conjunction]
    If the prompt is a conjunction of two questions $ p = (q_1 \wedge q_2, C) $, then the LLM is logically consistent if $ r(q_1 \wedge q_2, C) = r(q_1, C) \wedge r(q_2, C) $
\end{lemma}


\begin{example}
\normalfont
    \begin{align*}
        & q = \texttt{Which country is in South Asia and has a capital city called Delhi?}\\
        & q_1 = \texttt{Which country is in South Asia?}\\
        & q_2 = \texttt{Which country has a capital city called Delhi?}\\
        & q = q_1 \wedge q_2\\
        & C = \{\texttt{Bangladesh, India, Pakistan}\}\\
        & r(q_1 \wedge q_2, C) = \{\texttt{India}\} \\
        & r(q_1, C) = \{\texttt{Bangladesh, India, Pakistan}\} \\
        & r(q_2, C) = \{\texttt{India}\} \\
        &r(q_1 \wedge q_2, C) = r(q_1, C) \wedge r(q_2, C)
    \end{align*}
\end{example}

\subsection{Disjunction.}

\begin{lemma}[Disjunction]
    If the prompt is a conjunction of two questions $ p = (q_1 \vee q_2, C) $, then the LLM is logically  consistent if the following holds.
    \begin{align}
        r(q_1 \vee q_2, C) = r(q_1, C) \vee r(q_2, C)
    \end{align}
\end{lemma}


\subsection{Existential.}

\begin{lemma}[Existential]
    If the prompt is an existential \textbf{binary} question asking the LLM whether there exists any valid choice within the set of all choices, formally $ p = (q^{(\exists)}, C) $, then the LLM is logically consistent if the following holds.
    \begin{align}
        (q^{(\exists)}, C) = 
    \end{align}
\end{lemma}


\begin{example}[Existential]
\normalfont
    \begin{align*}
        & q^{(\exists)} = \texttt{Is there a country in \{Bangladesh, India, Germany\} which is in South Asia?}\\
        & C = \{\texttt{Yes, No}\}\\
        & q_{\mathsf{Ban}} = \texttt{Is Bangladesh in South Asia?}\\
        & C_{\mathsf{Ban}} = \{\texttt{Yes, No}\}\\
        & q_{\mathsf{Ind}} = \texttt{Is India in South Asia?}\\
        & C_{\mathsf{Ind}} = \{\texttt{Yes, No}\}\\
        & q_{\mathsf{Ger}} = \texttt{Is Germany in South Asia?}\\
        & C_{\mathsf{Ger}} = \{\texttt{Yes, No}\}\\\\
        & r(q^{(\exists)}, C) = \texttt{Yes} \\
        & r(q_{\mathsf{Ban}}, C_{\mathsf{Ban}}) = \texttt{Yes}\\
        & r(q_{\mathsf{Ind}}, C_{\mathsf{Ind}}) = \texttt{Yes}\\
        & r(q_{\mathsf{Ger}}, C_{\mathsf{Ger}}) = \texttt{Yes}\\
        & \Rightarrow r(q^{(\exists)}, C) = r(q_{\mathsf{Ban}}, C_{\mathsf{Ban}}) \vee r(q_{\mathsf{Ind}}, C_{\mathsf{Ind}}) \vee r(q_{\mathsf{Ger}}, C_{\mathsf{Ger}})
    \end{align*}
\end{example}


\begin{table*}
    \centering
    \caption{With context accuracy}
    \begin{tabular}{lrrr}
        \toprule
        Model & $ \mathbb{E}[\mathtt{LLM}(r(v_1, v_2)) = 1] $ & $ \mathbb{E}[\mathtt{LLM}(r(v_1, v'_2)) = 0] $ & Average\\
        \midrule
        Llama2 13B (chat) & $ 1.00 \pm 0.00 $ & $ 0.83 \pm 0.38 $ & $ 0.92 \pm 0.28 $ \\
        Llama2 7B (chat) & $ 0.99 \pm 0.09 $ & $ 0.81 \pm 0.39 $ & $ 0.90 \pm 0.30 $ \\
        \bottomrule
    \end{tabular}
    \vspace{1em}
    
    \caption{Without context accuracy}
    \begin{tabular}{lrrr}
        \toprule
        Model & $ \mathbb{E}[\mathtt{LLM}(r(v_1, v_2)) = 1] $ & $ \mathbb{E}[\mathtt{LLM}(r(v_1, v'_2)) = 0] $ & Average\\
        \midrule
        Llama2 13B (chat) & $ 1.00 \pm 0.05 $ & $ 0.02 \pm 0.14 $ & $ 0.51 \pm 0.50 $ \\
        Llama2 7B (chat) & $ 0.99 \pm 0.09 $ & $ 0.02 \pm 0.15 $ & $ 0.51 \pm 0.50 $ \\
        \bottomrule
    \end{tabular}
    \vspace{1em}

    \caption{Logical consistency with context.}
    \begin{tabular}{lr}
        \toprule
        Model & $ \mathbb{E}[\mathtt{LLM}(r(v_1, v_2)) \ne \mathtt{LLM}(r(v_1, v'_2))] $ \\
        \midrule
        Llama2 13B (chat) & $ 0.83 \pm 0.38 $ \\
        Llama2 7B (chat) & $ 0.80 \pm 0.40 $ \\
        \bottomrule
    \end{tabular}
    \vspace{1em}

    
    \caption{Logical consistency without context.}
    \begin{tabular}{lr}
        \toprule
        Model & $ \mathbb{E}[\mathtt{LLM}(r(v_1, v_2)) \ne \mathtt{LLM}(r(v_1, v'_2))] $ \\
        \midrule
        Llama2 13B (chat) & $ 0.02 \pm 0.15 $ \\
        Llama2 7B (chat) & $ 0.03 \pm 0.16 $ \\
        \bottomrule
    \end{tabular}
\end{table*}




==> checklist.tex <==


